Vis Ex Machina: An Analysis of Trust in Human versus Algorithmically Generated Visualization Recommendations

More visualization systems are simplifying the data analysis process by automatically suggesting relevant visualizations. However, little work has been done to understand if users trust these automated recommendations. In this paper, we present the results of a crowd-sourced study exploring preferences and perceived quality of recommendations that have been positioned as either human-curated or algorithmically generated. We observe that while participants initially prefer human recommenders, their actions suggest an indifference for recommendation source when evaluating visualization recommendations. The relevance of presented information (e.g., the presence of certain data fields) was the most critical factor, followed by a belief in the recommender's ability to create accurate visualizations. Our findings suggest a general indifference towards the provenance of recommendations, and point to idiosyncratic definitions of visualization quality and trustworthiness that may not be captured by simple measures. We suggest that recommendation systems should be tailored to the information-foraging strategies of specific users.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/abstract.tex <==
\begin{abstract}
%   More visualization systems are simplifying the data analysis process by automatically suggesting potentially relevant visualizations. However, little work has been done to understand if users trust these automated recommendations. In this paper, we present the results of a crowd-sourced study that explores preferences and perceived quality of human-curated versus algorithmically-generated recommendations. We observe that while participants initially prefer human recommenders, their actions suggest an indifference for recommendation source when evaluating visualization recommendations.
%   We found that the relevance of presented information (in terms of the presence of certain data fields) was the most critical factor, followed by a belief in recommender's ability (human or algorithm) to create accurate visualizations. 
%   Our findings suggest a general indifference towards the provenance of recommendations, and point to idiosyncratic definitions of visualization quality and trustworthiness that may not be captured by simple measures. We suggest that recommendation systems should be tailored to the information-foraging strategies of specific users.

More visualization systems are simplifying the data analysis process by automatically suggesting relevant visualizations. However, little work has been done to understand if users trust these automated recommendations. In this paper, we present the results of a crowd-sourced study exploring preferences and perceived quality of recommendations that have been positioned as either human-curated or algorithmically generated. We observe that while participants initially prefer human recommenders, their actions suggest an indifference for recommendation source when evaluating visualization recommendations. The relevance of presented information (e.g., the presence of certain data fields) was the most critical factor, followed by a belief in the recommender's ability to create accurate visualizations. Our findings suggest a general indifference towards the provenance of recommendations, and point to idiosyncratic definitions of visualization quality and trustworthiness that may not be captured by simple measures. We suggest that recommendation systems should be tailored to the information-foraging strategies of specific users.

\end{abstract}
   

%% Keywords that describe your work. Will show as 'Index Terms' in journal
%% please capitalize first letter and insert punctuation after last keyword
\keywords{Visualization recommendation systems, algorithmic trust, automation, recommendation source}

%% ACM Computing Classification System (CCS). 
%% See <http://www.acm.org/class/1998/> for details.
%% The ``\CCScat'' command takes four arguments.

%\CCScatlist{ % not used in journal version
% \CCScat{K.6.1}{Management of Computing and Information Systems}%
%{Project and People Management}{Life Cycle};
% \CCScat{K.7.m}{The Computing Profession}{Miscellaneous}{Ethics}
%}

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/acknowledgements.tex <==
\section{Acknowledgements}
We thank all the reviewers, study participants, and members of both the Human-Computer Interaction Lab and the Battle Data Lab for their valuable feedback. 

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/analysis.tex <==
% \usepackage[table,xcdraw]{xcolor}
\section{Analysis}
\label{sec:analysis}

In this section, we investigate our research questions via a mixture of quantitative and qualitative methods, focusing our analysis on the link between participants' prior preferences regarding recommendation sources, the participants' measured relevance of the displayed visualization panels, and their self-reported rationales for choosing one panel of visualization recommendations over another.

%\vspace{-3mm}
\subsection{Preliminaries}
In this section, we define specific concepts and calculations used throughout our analysis, and summarize our analysis methods. We compute panel relevance based on a fixed set of attributes collected in a pilot study, as well as by using participants' top five selected attributes (see \autoref{sec:experiment-design:relevance} and \autoref{sec:experiment-design:limitations}). The specific relevance measures we analyze are as follows:

\begin{description}[nosep]
  \itemsep0em
 \item[\emph{A Priori} or Participant Ranking] The ranking of the five most frequently selected attributes from our pilot study or by a specific participant respectively. 
%  \item[\emph{A Priori} Relevance] The computed relevance for each of our four recommendation panels, with respect to the a priori ranking.
%  \item[Participant Ranking] The top five attributes selected by a specific participant. 
%  \item[Relevance] The relevance score for a given panel using the participant ranking instead of the a priori ranking. 
\end{description}

% We collected various measures in our experiment to gauge how participants perceived the relevance and quality of recommendation panels, which we review here.
%(see \autoref{sec:experiment-design} for experiment details):
\begin{description}[nosep]
 \item[Panel Rating] The rating that a participant assigned to a specific panel, using a ten point Likert scale. 
 \item[Attribute Overlap] Given two sets of attributes, we calculate the cardinality of the intersection of the two sets.
 %Each panel represents a corresponding set of attributes, and each participant builds a ranked list of attributes that can be compared.

%  \item[Chosen Panel] Given a pair of panels reviewed by the participant, the specific panel that the participant selected for further analysis. 
%  \item[Unchosen Panel] The panel that was \emph{not} selected by the participant.
\end{description}
Note that each recommendation panel (and individual visualization within this panel) represents a unique subset of attributes, which may or may not overlap with a user's preferred attributes.
% We also distinguish between participants who are consistent versus inconsistent with their recommendation preferences:
% \begin{description}
%  \item[Adherent] .
% %  \item[Defector] A participant who deviates from their prior recommendation preference. %(i.e., prior preference was for human recommendations, but selected the ``Algorithmically-Generated'' panel).
% \end{description}

\subsubsection{Quantitative Analysis Methods Overview}
\label{sec:analysis:exploratory-analysis-overview}

Our quantitative measures aim to uniformly assess the decisions made by participants, such as the frequency of \highlight{when} each source was selected or the distribution of ratings assigned to each recommendation panel.
%Our main quantitative measures were the explicit choices made by the participants, their ratings associated with those choices, and the calculated relevance of the panels.
Given the context of our study design and tentative hypotheses, we also opted for a more exploratory rather than confirmatory design for analyzing our study data. Rather than relying on inferential statistical analysis, we used our quantitative analysis to identify patterns in participants' visualization preferences and analysis behaviors, and report on general effect sizes and confidence intervals to provide additional context for our findings.

% We did not feel that existing measures for trust or visualization recommendation quality were mature enough to directly apply to our cases of interest. Similarly, the breadth of our exploration did not seem well suited to the more depth-first approach of inferential statistical analysis. Therefore, we used our quantitative analysis to identify patterns in participants' visualization preferences and analysis behaviors, and report on general effect sizes and confidence intervals to provide additional context for our findings.

\subsubsection{Qualitative Analysis Methods Overview}
\label{sec:analysis:qualitative-analysis-overview}
In our experiment, we explicitly asked participants to explain their choice in recommendation panel (see \autoref{sec:experiment-design:comparing}). These responses form the basis for our qualitative analysis. We note that two responses were excluded from the analysis. One response was not written in English, preventing an accurate evaluation, and the other was empty. We qualitatively coded 112 responses for this analysis.

We performed open coding~\cite{lazar2017research} on participants' free text responses explaining the reasons for their panel selection; the codes are provided in \autoref{tab:codes}.  To develop a consistent coding scheme, two researchers coded the first 40 responses individually, then discussed to resolve discrepancies.
%For example, we initially disagreed upon how to code the following response: 
%\begin{quote}
%prefered the content analysed in the human-curated data. I feel it is more useful in gauging consumer interest for a movie and the likelihood of its success
%\end{quote}
%One researcher assigned the code "trust in humans," because the implication seemed to be that humans are better at understanding consumers' interests. However, we decided that "trust in humans" did not apply to this particular response, because the participant's judgment pertained to the usefulness of the panel rather than ability of humans to create visualizations.
One researcher coded the remaining responses, which the other reviewed. We used a multi-phase coding process to refine and merge similar codes. Then, the resulting 24 codes were organized into six high-level themes describing the reasoning behind participants' decision-making processes.

\begin{comment}
\begin{table}[]
\begin{tabular}{|p{3cm}|p{6cm}|}
\hline
\textbf{Term} & \textbf{Definition} \\ \hline
relevance & \begin{tabular}[c]{@{}l@{}}The relevance score calculated from \\ the participant's ranking of the top 5 attributes.\end{tabular} \\ \hline
a priori ranking & \begin{tabular}[c]{@{}l@{}}The overall top 5 attributes identified in \\ the pilot study\end{tabular} \\ \hline
a priori relevance Score & \begin{tabular}[c]{@{}l@{}}The relevance score we assigned to the panels,\\ calculated from the a priori ranking\end{tabular} \\ \hline
Panel Rating & \begin{tabular}[c]{@{}l@{}}Likert score indicating the helpfulness of \\ the panel, where 1 is not at all helpful and \\ 10 is extremely helpful.\end{tabular} \\ \hline

Chosen Panel & \begin{tabular}[c]{@{}l@{}}The panel that a participant selected to use \\ for further analysis\end{tabular} \\ \hline
Unchosen Panel & \begin{tabular}[c]{@{}l@{}}The panel that a participant did not select to use \\ for further analysis\end{tabular} \\ \hline
Attribute Overlap & \begin{tabular}[c]{@{}l@{}}The number of attributes in common between \\ the participant's top 5 ranked attributes and \\ the attributes displayed within a given \\ recommendation panel. The range of common \\ attributes will necessarily be between 1 and 5.\end{tabular} \\ \hline
Defector & \begin{tabular}[c]{@{}l@{}}Participants that expressed a preference for \\ one type of recommendation, but chose another. \\ For example, a participant that expressed a \\ preference for human recommendations, \\ but chose an algorithmically-generated \\ recommendation panel.\end{tabular} \\ \hline
Adherent & \begin{tabular}[c]{@{}l@{}}Adherents are participants that expressed a \\ preference for one type of recommendation \\ and stuck with that recommendation type.\end{tabular} \\ \hline
\end{tabular}
\caption{All of the terms later used in our analysis}
\label{tab:terminology}
\end{table}
\end{comment}

%\vspace{-3mm}
\subsection{Verifying Recommendation Relevance}
\label{sec:analysis:relevance}
Before evaluating the effects of recommendation source preference on decision-making, we assess the alignment between participants' perceptions of panel relevance and our calculated relevance scores. This analysis serves to not only anchor our measures, but also to explore our first hypothesis -- that people will rate recommendation sources according to the degree of attribute overlap. Our results are as follows:

%In this section, we discuss our approach and findings when comparing a priori relevance measures to new ones adjusted for participants' attribute preferences. 

%We first analyzed attribute overlap to determine commonalities between our expectations of relevant features and those of participants. Then, we focused on relevances and panel ratings to explore correlations with our relevance metrics. The results of this analysis indicate that our measures of relevance were corroborated by users' perceived relevance.

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.65\linewidth]{figures/histogram_us_them_top5.png}
%     \caption{Distribution of attribute overlap for a priori rankings and participant rankings.} 
%     \label{fig:histogram_us_them_top5}
%     \vspace{-4mm}
% \end{figure}

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.65\linewidth]{figures/user_panel_relevance.pdf}
%     \vspace{-3mm}
%     \caption{Distribution of relevances by panel ID. HR1 refers to the first high relevance panel, and LR1 refers to the first low relevance panel. Participants rated all panels as generally similar in relevance, regardless of number of relevant features included in the panel.
%     }
%     \label{fig:user_based_relevance_per_panel}
% \end{figure}

\textbf{A priori rankings have high attribute overlap with participant rankings}:
We first analyze attribute overlap between a priori and participant rankings, shown in \autoref{fig:figure1}, where the range of attribute overlap is from 0 (i.e. no overlap) to 5 (i.e. both sets are identical).
We find similarities between a priori and participant rankings. 70\% of participants selected at least three of the same attributes used in the a priori rankings. This indicates that our a priori relevance seems to be aligned with participant relevance, and thus was a reasonable starting point for generating high- and low-relevance panels.

%\astha{As a result, our panel relevance metric (see \autoref{sec:experiment-design:relevance}) yields similar results when substituting a priori for participant rankings (Pearson R correlation of 0.31). }

% Moreover, when calculating the distribution of relevance scores for each panel and participant, shown in \autoref{fig:user_based_relevance_per_panel}, we find that low-relevance panels tend to also have lower participant relevance scores. Thus, a priori relevance seems to be in general alignment with participant relevance, and was a reasonable starting point for generating high- and low-relevance panels.

%Because the panels generally contain three or more features of interest, we have now established a baseline relevance for the panels on the whole, setting the stage for further analysis of the perceived relevance of the panels. 




% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/figures_1.png}
%     \caption{Figure 4 is   \leilani{I would use a subfigure package rather than cramming the figures into the same image, subcaption would be an example.}}
%     \label{fig:figures_1.png}
%     \vspace{-3mm}
% \end{figure}

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.65\linewidth]{figures/user_panel_ratings_by_common_features.pdf}
%     \caption{Distribution of panel rating by number of common features, or attribute overlap.}
%     \label{fig:panel_rating_by_total_attribute_overlap}
%     \vspace{-3mm}
% \end{figure}

% (Astha) to me, this seems like an obvious byproduct of having similar fixed / participant rankings so I'm not sure if this needs to be it's own paragraph, but instead can be lumped up with the above one
% \textbf{a priori relevance scores seem to align with relevances}:
% To assess whether our panels are actually perceived as having relatively higher and lower relevance, we calculate the distribution of participant responses for each panel and compare them. First, we calculate the relevance for each panel and participant, shown in \autoref{fig:user_based_relevance_per_panel}. The low-relevance panels are colored green, the high-relevance panels blue. Though there is wide variation in the scores, we still see a trend where the low-relevance panels tend to also have lower relevances. Thus, our fixed scores seem to be in alignment with our relevances, consistent with our first hypothesis.
  
%(Astha) Because we don't really talk about this much later on, I feel like it's better to condense the relevance metrics section. The relevance metrics aren't our major contribution anyway.      
% \textbf{Raw panel ratings alone is not a strong indicator of relevance}:
% To understand whether participants themselves rate the panels as higher or lower relevance, we compare participants' panel ratings across our four panels, shown in \autoref{fig:panel_rating_per_panel}.
% %We then analyzed user panel ratings to directly evaluate participants' perceptions of panel relevance.
% We see that there are only minor differences between the panel ratings of low relevance and high relevance panels, suggesting that participants tend to rate them similarly. This is further confirmed when analyzing panel ratings based on attribute overlap between the panel and participant rankings, we find a similar result (see \autoref{fig:panel_rating_by_total_attribute_overlap}). Participants seem to assign a very similar range of scores when there are very few overlapping attributes as when there are many overlapping attributes; this result can be seen by comparing the first and last boxplots in \autoref{fig:panel_rating_by_total_attribute_overlap}.
% Therefore, we find that Panel Ratings alone do not appear to be a strong signal for gauging the absolute relevance of the panels.
%\autoref{fig:panel_rating_by_total_attribute_overlap} furthers this by comparing user panel relevance with attribute overlap. Though attribute overlap has been shown to be a good indicator of relevance, there is no discernible difference between median panel ratings and attribute overlap. Despite this, relative differences in assigned ratings may still be significant. 

\textbf{Participants seem to emphasize relative rather than absolute panel ratings}:
% To understand whether participants themselves view the panels as higher or lower relevance, we compare participants' panel ratings across our four panels, shown in \autoref{fig:panel_rating_per_panel}.
%We then analyzed user panel ratings to directly evaluate participants' perceptions of panel relevance.
% \astha{If we later need space, a candidate figure to remove would be Figure 6}
% As attribute overlap seemed to correlate with perception of utility, we analyzed panel ratings across attribute overlap.
%\astha{Participants seem to assign a very similar range of scores irrespective of the number of overlapping attributes; Attribute Overlap and Rating has a Pearson R of 0.1, implicating that participants see them as being of equal value (see \autoref{fig:figures_2}). }
%We found similar results when outright comparing participant panel rating by panel IDs.

Participants rated the presented panels similarly. However, since participants were asked to compare \emph{pairs} of panels rather than panels in isolation, it is possible that participants are focusing on \emph{relative} differences when assigning ratings to panels. 
%Because the analysis task involves examining both panels side by side and then making a choice, it is important to examine whether differences in panels are indicative of differences in user ratings.
%Suppose a participant perceives panel A as being more relevant than panel B; then the participant may assign A a higher rating than B (e.g., a score of seven versus six). Even though the scores of A and B are very similar, it is the \emph{difference} in score that is more important.
%This effect could be observed by calculating differences in attribute overlap (which appears to be a useful indicator of relevance), and comparing with positive-negative differences in participants' panel ratings.
To evaluate this scenario, we first compare each panel to the corresponding ranking assigned by each participant. One panel will overlap more or equally with the participants' rankings than the other. Subtracting the lower overlap value from the higher produces a new value between zero and five. We then apply the corresponding calculation for panel ratings: subtracting the rating of the low-overlap panel from the rating of the high-overlap panel.
\autoref{fig:figures_2} illustrates the results, where the x-axis represents the difference in attribute overlap for a pair of panels, and the y-axis represents the corresponding difference in panel ratings. The figure illustrates a trend where as the difference in attribute overlap increases, so does the difference in panel rating. This suggests that participants may view relevance as a function of attribute overlap, and so rating alone may not be sufficient to describe the perceived utility of a panel. Thus, the panel ratings may be useful in terms of measuring \emph{relative} preference between a given pair of recommendation panels. 
% Bubble size encodes the number of participants that assigned the corresponding relative score (i.e., score difference).
%further examines this by visualizing the differences in user panel rating against the differences in overlapping attributes. In particular, the y-axis is the difference between the panel rating of the panel with a higher attribute overlap  and the panel rating of the panel with a lower attribute overlap.
%The size of the bubbles represent algorithmically scaled frequency. 
%\astha{The positive upward trend suggests that participants do notice when one panel contains more attributes of interest, and will assign a relatively higher score to this panel (Pearson R of 0.75 ) . Participants appear to rate recommendation source on overlap.} 

% This supports our first hypothesis, where participants appear to rate recommendation source based on attribute overlap. 

%The positive upward trend seems to indicate that participants' perceptions of relevance are relatively aligned with the attribute overlap.

% \textbf{Participants rate chosen panels higher than unchosen ones}: To see whether participants actually do rate their preferred panels higher than other panels, we compare the ratings for panels that were selected by each participant (or \emph{chosen} panels) to those that were not selected (\emph{unchosen} panels), shown in
% \autoref{fig:panel_rating_by_selection_status}.
% We find that participants do tend to rate chosen panels more highly,
%We find that participants tend to select panels that they rate more highly, with the median panel rating for chosen panels being higher than for unchosen panels.

\begin{figure}
\centering
\begin{minipage}[t]{0.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/rating_by_attribute.pdf}
\subcaption[first caption.]{A distribution of panel rating by attribute overlap: the number of data features selected as relevant by the participant that appear in a particular panel of recommendations. Bars represent 95\% confidence interval with 1000 bootstrapped iterations.}
\Description{Swarm plot of panel ratings, separated by attribute overlap. Despite different levels of attribute overlap, participants generally rated panels similarly.}
\end{minipage}
\begin{minipage}[t]{0.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/diff_feature_overall_likert.png}
\setlength{\belowcaptionskip}{-8pt}

\subcaption[second caption.]{
As comparatively more data fields selected by the participant as relevant appear in a panel of recommendations, the subjective rating of the chosen panel likewise increases. The y-axis is the comparative difference in rating between chosen and unchosen panels. The x-axis is the difference in attribute overlap between the chosen and unchosen panels, and the
% \highlight{\sout{y-axis is the number of responses. The} } 
radius is the number of responses.
}\label{fig:figures_2}
\Description{Bubble plot with the absolute difference in panel ratings vs absolute differences in attribute overlap. Bubble size encodes the number of participants with the corresponding score difference. There is an upward trend indicating that participants are giving increasingly different ratings when the panels exhibit increasingly different levels of attribute overlap.}
\end{minipage}
\setlength{\belowcaptionskip}{-8pt}

\caption{Relative difference appears to be a better metric than absolute difference.}\label{figures_1.png}
\end{figure}

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/figures_2.png}
%     \vspace{-3mm}
%     \caption{\mc{Weren't we going to make B a beeswarm? Also we only talk about Figure A in this caption, but both A and B are important.}Figure A is } 
%     \label{fig:figures_2}
%     \vspace{-3mm}
% \end{figure}
%  \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.65\linewidth]{figures/diff_feature_overall_likert.png}
%     \vspace{-3mm}
%     \caption{Absolute difference in panel ratings vs absolute differences in feature overlap. Bubble size encodes the number of participants that assigned the corresponding relative score (i.e., score difference)} 
%     \label{fig:difference_panel_rating_attribute_overlap}
%     \vspace{-3mm}
% \end{figure}

 
 %(Astha) Let's move these summaries into the discussion   
% \textbf{Relevance analysis summary}:
% We find that our a priori rankings and a priori relevance scores seem to align with participants' attribute rankings and relevances. To evaluate whether participants actually perceive our high-relevance panels as being more relevant compared to the low-relevance panels, we analyze participants' panel ratings. We find that the \emph{relative difference} in ratings for a given pair of panels appears to matter more than the actual ratings themselves.
% Taken all together, these findings seem to suggest that \textbf{our a priori relevance scoring mechanism is in alignment with participants' perceptions of panel relevance.}
% %Taken together, these findings support the continued usage of our relevance metric as a measure of user-perceived relevance.

% Furthermore, we find that participants seem to ascribe higher ratings to and ultimately select recommendation panels that overlap more with their attribute ratings. Thus, our results seem to suggest that \textbf{participants prioritize visualization recommendations by attribute relevance}, supporting hypothesis \textbf{H1}.

%\vspace{-3mm}

% \subsection{Assessing Bias in Participant Preferences and Panel Selections}
% \label{sec:analysis:bias}



% our relevance metrics appear to correlate with participant-based relevance metrics.

\begin{table*}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Themes} & \multicolumn{4}{l}{\textbf{Codes}} \\ \hline
Data-driven Decisions (60) & \multicolumn{4}{l}{Information quality (11), information usability (25), relevance (5), visualizations of interest (23), attributes of interest (27)} \\ 
Trust in Source (22) & \multicolumn{4}{l}{\begin{tabular}[c]{@{}l@{}}Trust in ability of humans or algorithm (19), human touch (3), trust in dataset (1), desire for insight on recommender's process (1)\end{tabular}} \\ 
Reliability of Source (21) & \multicolumn{4}{l}{Reliability (11), accuracy (10), errors (4)} \\ 
Participant Comprehension (17) & \multicolumn{4}{l}{Comprehension (16), ease of analysis (2)} \\ 
Personal Experiences (16) & \multicolumn{4}{l}{\begin{tabular}[c]{@{}l@{}}Personal preference (6), personal background (3), preference for a data representation (3), indifference (2)\end{tabular}} \\ 
Visual Aesthetics (7) & \multicolumn{4}{l}{Visual aesthetics (7), color preference (1)} \\ \hline
\end{tabular}
}
\caption{The codes derived from our qualitative analysis, organized by high-level themes. }
\Description{A 2 column table, with the first column containing all of the themes from our qualitative analysis and the frequency of occurrence. The second column contains the codes associated with that theme, as well as their frequency of occurrence. The 6 themes are Data-driven decisions, Trust in Source, Reliability of Source, Participant Comprehension, Personal Experiences, and Visual Aesthetics.}
\label{tab:codes}
\end{table*}

\subsection{Assessing Bias in Participant Preferences and Panel Selections}
\label{sec:analysis:bias}

%In this section, we explicitly address our research questions, in particular \textbf{RQ1} and \textbf{RQ2}. 

% In this section, we investigate whether participants exhibit preferences or selection behaviors biased towards specific sources of visualization recommendations (human or algorithms).

In this section, we explore our first research question:
\emph{How do existing preferences for human-curated versus algorithmically-generated recommendations affect the evaluation of recommendation quality or utility?} This  will also help us explore our second hypothesis -- \emph{that an a priori preference towards a particular recommendation source predisposes participants to select a particular panel, regardless of recommendation relevance.} 

%We provide additional context for our quantitative results through a qualitative analysis of participants’ free-text responses regarding the reasons for their panel selections. 

\textbf{Though participants initially prefer human recommendations, they are neutral to source in their panel selections}: First, we delved into understanding the existing preferences and subsequent decisions made by our participants. 60\% indicate a prior preference for human recommendations, 15\% prefer algorithmic recommendations, and 25\% have no preference. Though this suggests an existing preference for human recommendation sources, \highlight{participants'} subsequent recommendation source choices are evenly split between humans and algorithms (see \autoref{fig:sankey}).

\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/sankey.png}
    \setlength{\belowcaptionskip}{-8pt}
    \caption{Sankey diagram of prior preferences of recommendation sources and posterior selection of panels. Most people expressed a prior preference for human sources, but the resulting posteriors are split nearly 50/50}
    \label{fig:sankey}
    \Description{Sankey diagram of prior preferences of recommendation sources and posterior selection of panels. Most people expressed a prior preference for human sources, but the resulting posteriors are split nearly 50/50}
\end{figure}

\textbf{Prior preferences are not highly predictive of visualization recommendation choices:} For participants who initially \highlight{preferred} human recommendations, 58\% \highlight{selected} the ``Human-Curated'' panel. For participants who initially \highlight{preferred} algorithmic recommendations, 59\% \highlight{selected} the ``Algorithmically-Generated'' panel. 62\% of participants with no initial preference selected the ``Algorithmically-Generated'' panel. Given that we controlled for relevance across all conditions, these findings suggest that participants \highlight{did} not primarily select panels based on their a priori preference for human or algorithmic recommendations. Nevertheless, there was a subset of participants that did not follow this trend.  
 
% These results support our findings in \autoref{sec:analysis:relevance} in that a majority of participants’ panel selection choices appear to be driven by the perceived relevance of the data attributes represented in the corresponding visualizations.

%where relevance was not the only explanation for panel selection.



%Now, we focus on the cases where participants adhere to their priors, even when the chosen panel is \emph{less} relevant, which could potentially indicate existing bias. We define an adherent as a participant who selects the recommendation panel that is consistent with their prior recommendation preference (i.e., their prior preference was for human recommendations, and they selected the ``Human-Curated'' panel). 43 of 112 participants were classified as adherents. We find that 36.7\% of all adherents (and thus 14\% of all participants) stick with their prior preferences, even when the relevance of the chosen panel is lower than that of the unchosen panel. Though far from a majority, this result may suggest that some participants may still make allowances for their preferred recommendation source, and thus may be susceptible to recommendation errors. However, it is also possible that these adherents have different preferences for visualization recommendations (i.e., our relevance calculations do not align with how these specific participants perceive relevance). We qualitatively explore alternative measures of relevance from participants in the next section.

% Now, we focus on the cases where participants adhere to their priors, even when the chosen panel is \emph{less} relevant, which could potentially indicate existing bias. 
% We define an adherent as a participant who selects the recommendation panel that is consistent with their prior recommendation preference (i.e., their prior preference was for human recommendations, and they selected the ``Human-Curated'' panel). 
\textbf{A fraction of adherents chose their panel despite estimated lower relevance}: We find that 14\% of all participants stick with their prior preferences, even when the calculated relevance of the chosen panel is lower than that of the unchosen panel (average relevance of chosen of 8, unchosen is 11). Though far from a majority, this result may suggest that some participants may still make allowances for their preferred recommendation source, and thus may be susceptible to recommendation errors.

It is possible that our relevance metric did not align with how these specific participants' models of relevance. Our metric was calculated using participants' attribute rankings only, and does not account for interaction effects between attributes or other potential indicators of utility. As a result, we qualitatively explore alternative measures of relevance from participants in the next section.

% Based on these findings, we can address our first research question: participants' preferences for recommendation source seems to largely be driven by the relevance of the information within the recommendations themselves. 
In summary, though our participants initially appeared to have preferences for human recommendation sources, they were ultimately neutral to visualization recommendation sources. However, there is a minority of people that appear to make allowances for their prior preferences, which may drive their choice of recommendation source. 
%This result contradicts our second hypothesis.
% where we expected participants to exhibit bias towards their preferred recommendation source.
% 

\subsection{Understanding Participants' Decision Making Models}

After observing that most participants claim to prefer human recommendations yet in practice are insensitive towards recommendation source, we explore our second research question: \emph{If clear preferences are observed, what reasons do users give for preferring a certain recommendation source?} We qualitatively analyze participant responses to understand their reasoning for choosing a certain panel.

\textbf{Many participants reported selecting panels in an analysis-driven way}: The most common theme (60 out of 112 responses) was analysis-driven decisions, meaning that participants evaluated panels based on their own analysis interests and the corresponding applicability of the information encoded within the visualizations. Within that umbrella category, participants fell into different clusters of reasoning. Some participants seemed to regard each panel as a whole and chose a panel based on the combined utility of the component visualizations. As an example, one participant noted: 
% \vspace{-2mm}
\begin{quote}
    \emph{Although the selection doesnt reflect all of the attributes picked earlier on, i think the data in this set matches more so what i want to focus on in the pitch. (P91)}
\end{quote}
\vspace{-1mm}
These participants seem to suggest that they prioritized the cumulative information gained when choosing one panel versus the other.
%These participants appear to note the ability of multiple visualizations to aid in creating their pitch.
On the other hand, there were participants who noted specific visualizations or attributes that swayed their decision to choose a particular panel, and thus recommendation source. In particular, 19 of these 60 participants mention specific visualizations within their justification. For example, one participant wrote: 
\vspace{-1mm}
\begin{quote}
    \emph{[the] last bit of human curated (domestic gross v release year) was really convincing chart (P33)}
\end{quote}
\vspace{-1mm}

Lastly, many participants expressed interest in specific attributes or visualizations, situated with respect to the context of their movie pitches. For example, another participant stated:
\vspace{-1mm}
\begin{quote}
\emph{[the] algorithmically-generated grid has some very useful graphs, such as profit/mpaa rating and budget/genre...the company that the movie is being pitched to would be really interested in these particular sets of data. (P54)}
\end{quote}
\vspace{-1mm}
Overall, even within the data-driven decisions theme, there was a significant diversity in rationales, be it the combined utility of visualizations, a singular visualization, or focusing on potentially interesting attributes for the target audience.

\textbf{Trust in the source of recommendations was the second most common reason for choosing a particular panel}. In examining adherents in \autoref{sec:analysis:bias}, we became interested in understanding the potential biases people harbor towards a particular recommendation source. We observed the theme ``Trust in Source'' in 22 of 112 responses. %Trust in source describes the level of trust that a participant had in the source of recommendations (22 of 22 responses),
%be it the algorithm or the human-curator,
%as well as why the participant trusts or distrusts this source (21 of 22 responses).

Some participants believed that algorithms are more efficient and less likely to make errors than humans (6 of 22 responses). As P75 explained, 
\vspace{-1mm}
\begin{quote}
   \emph{``Although they [the panels] both seemed equally helpful to me, I chose the algorithmical one because human curated may have some mistakes in it but algorithmical one most probably does not.''}
\end{quote}
\vspace{-1mm}

This reasoning came from a general impression that algorithms are more accurate, or from the participant's personal background, as one participant notes: \emph{...I inhere[n]tly tend to trust Algorithms more since I am a computer s[c]ience student. (P97)}

Conversely, some participants indicated a preference for humans due to the presence of a ``human touch'' in the recommendation panels (3 of 22 responses). For example, one participant
references this notion of a uniquely human quality in the human-curated visualizations by explaining that
\vspace{-1mm}
\begin{quote}
   \emph{``Both [panels] had good information but I think the human touch is required to get the best feel for the data'' (P65).} 
\end{quote}
\vspace{-1mm}
Along a similar vein, one participant made their choice based upon the notion that \emph{because} a human recommended these visualizations, it had intrinsic value:
\begin{quote}
\emph{``I prefer things made by actual people and not algorithms, although the later could be useful too'' (P94)}
\end{quote}
\vspace{-1mm}
%\vspace{-2mm}
%\begin{quote}
    %\emph{I think it would be more interesting to understand why a person selected some charts for a grid. (P27)}
%\end{quote}
%\vspace{-2mm}
When both recommendation options are perceived as equally relevant, factors outside of the data relevance become increasingly important. Some participants will incorporate prior preferences for algorithmic or human recommendations into their decision making process. In the case of participant P65, the ``human touch'' becomes the deciding factor in selecting the ``Human-Curated'' panel. For participant P75, it was the added legitimacy and accuracy that an algorithm lends to recommendations. 

\subsection{Exploring How Analysis Experience And Other Factors Influence Participant Preferences}
%It was interesting to note that there were other factors affecting participants' evaluation strategies that are not directly tied to the relevance of the data or recommendation source.
Given the wide range of factors that could affect a participant's evaluation strategies, we seek to better understand how data analysis experience may influence how these factors are prioritized by participants.
In this section, we explore our third research question: \emph{What effect (if any) does statistical or data analysis experience have on user preferences?}

\textbf{Analysis experience does not seem to impact prior preference or panel selections}:
We recorded four measures of data analysis experience: statistics, visualization, general data analysis, and data analysis tool (Excel, R, Matlab, etc.) experience. For all measures, we failed to find a notable difference across experience levels. For sake of space, we only present a single salient example.  
% For this measure, we record roughly how often people perform data analysis tasks: almost never, less than monthly, less than weekly, and daily.
We \highlight{found} that participants selected the ``Algorithmically-Generated'' panel at similar rates regardless of frequency of performing data analysis tasks, used as an indicator for general data analysis experience level: 55\% (almost never), 53\%(less than monthly), 50\% (less than weekly), 33\%(weekly), and 67\% (daily). Thus, data analysis experience does not appear to be predictive of panel selection, answering our third research question. 

\textbf{Visualization comprehension may affect participants' ability to evaluate recommendations}: Despite this, a notable number of responses were categorized under ``Participant Comprehension'' (17 of 112 responses).
%The notion of a panel being more comprehensible or easy to understand appears in 17 of 112 responses. 
In particular, we find that some participants had trouble interpreting the visualizations in some of the panels. For example, one participant mentions that \emph{``the ones with the little dots are very confusing'' (P61).} This issue touches on one of the limitations of our experiment design (see \autoref{sec:experiment-design:limitations}), and poses a challenge for recommendations in general: not everyone values the relevance of a recommendation in the same way, and relevance can mean different things for users of differing levels of experience. For example, novice users may prioritize comprehension and ease of understanding, whereas more experienced users may prioritize insight density.

% This issue touches on one of the limitations of our experiment design (see \autoref{sec:experiment-design:limitations}), and poses a challenge for recommendations in general: not everyone comes to visualizations with the same level of experience, which may affect their ability to evaluate recommendation quality and relevance.

\textbf{Aesthetics can be a deciding factor in choosing between visualization recommendation panels}: The aesthetics of visualizations also seems to be a relevant factor in judging recommendations. Seven of 112 responses contained the  ``Visual Aesthetics'' theme, which refers to the artistic appearance of the visualizations themselves. Two participants cited the ``cleanness'' and ``simplicity'' of certain panels as the reasons for their selections. One participant in particular selected their chosen panel because the \emph{``blue color is visually more impactful'' (P55).} These sorts of design choices are often overlooked in making recommendations, to the detriment of users who value them.

%In computer science, we often strive to reduce subjectivity in algorithmic decision making. However, factors such as aesthetics and visual appeal may be devalued in this process to the detriment of users who value them.
%However, amongst the general population, it can still be a prioritized factor, and in some cases, a determining factor.


%\textbf{Panel ratings are still very similar across sources}:
%To further assess whether participants perceive recommendations differently across sources, also compare panel ratings by priors and panel selections (see \autoref{fig:panel_priors}). We find that participants tend to ascribe similar ratings to panels, regardless of source. However we do observe a slight increase in ratings for participants who initially prefer and ultimately select human-curated recommendations.%furthers this observation, by noted that participants' prior preferences did not have an effect upon panel rating for a given panel.

Based on these findings, we summarize how participants seem to choose between panels: participants often approach the evaluation of visualization recommendations in an analysis-driven way, but an inherent trust in recommendation source may play a role as well. For some, comprehension and visual aesthetics were also notable determining factors in selecting specific recommendation panels.

%Participants who indicate that they ``almost never'' perform data analysis tasks had a prior preference for human recommendations 54.5\% of the time, but selected the algorithmically-generated grid 54.5\% of the  time. All participants who perform data analysis on a daily basis had no prior preference, and were also more likely to select the algorithmically-generated grid (66.7\%). Interestingly, participants who perform weekly data analysis had a human prior preference 61.9\% of the time and selected the human grid 66.7\% of time. 


%analyzed understand reasoning for grid choices 
% better understand 50 50%
% Higher Relevance was driving factor


% \textbf{Bias Analysis Summary}:
% Overall, we find that participants begin the experiment with a modest preference for human-curated recommendations. However, as participants evaluate recommendations and choose between panels, we find that this initial bias effectively disappears. 
% These findings also appear to be consistent with our previous relevance analysis: participants generally seem to ascribe higher ratings to and select panels that are more relevant, where in our experiment design, relevance is independent of recommendation source.

% Though far from the majority, we do find that a notable fraction of participants stick with their preferred recommendation source, even when it turns out that the corresponding panel is less relevant, partially supporting hypothesis \textbf{H2}.

% Based on these findings, we can address research question \textbf{Q1}: existing recommendation preferences generally seem to have little effect on how participants rate and select visualization recommendations. 
% Furthermore, our results seem to suggest that participants' data analysis experience do not effect their prior recommendation preferences or panel selections, addressing research question \textbf{Q2}.
% However, a fraction of participants may still be susceptible to recommendation bias.

%\vspace{-3mm}




%Specific for question Q50
%Removed non english and incomplete (112 responses analyzed) 
%Example of disagreement 
%\vspace{-3mm}


%\vspace{-2mm}

%For example, some of the initial codes clustered underneath the %umbrella theme of "Data Analysis Process" include the relevance %of the data, the usability of the information within the pitch, % and the desire to examine specific charts and trends. 




% \textbf{Qualitative Analysis Summary}:
% Overall, our qualitative analysis illustrates a variety of reasons for selecting a specific visualization recommendation panel. We find that for a majority of participants, their decision-making process often focuses on the relevance of the data itself. However, some participants also explicitly mention trust in a specific recommendation source, indicating that prior preferences (and therefore biases) may play a role in subsequent decision-making. Several participants were swayed by the visual aesthetics of the panels. For some participants, challenges in interpreting certain visualizations may hinder their ability to effectively evaluate recommendation panels.



==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/conclusion.tex <==
\section{Conclusion}
As visualization systems increasingly rely on automated or semi-automated methods, and as the population of people who encounter visualization tools becomes larger and less specialized, the attitudes and beliefs of our users towards algorithmic recommendations will become increasingly important. The results of our experiment show that, for the most part, people seem to assess visualization recommendations in terms of relevance, rather than source; this seemed to hold across groups of varying statistical experience. However, there was a minority of people who did not seem to act in a data driven way. For instance, visual comprehension and aesthetics choices seemed to drive the decision-making of some participants, who should also be considered when designing large-scale systems. In that way, people are (with some exceptions) generally capable of adjusting their beliefs about the source of recommendations to fit their analytical needs, and making informed decisions about what recommendations to trust.

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/design.tex <==
\section{Experimental Design}
\label{sec:experiment-design}
\begin{table*}[tb]
\begin{tabular}{l l}
\hline
\textbf{Attribute Category} & \textbf{Attribute Names}                              \\ \hline
\textbf{Ratings}            & \begin{tabular}[c]{@{}l@{}}IMDB Vote Average (Q), IMDB Vote Count (Q)\end{tabular}                                                                    \\ \hline
\textbf{Finances}           & \begin{tabular}[c]{@{}l@{}}Budget (Q), Domestic Gross (Q), Profit (Q), Worldwide Gross (Q)\end{tabular}                                                \\ \hline
\textbf{Details}            & \begin{tabular}[c]{@{}l@{}}MPAA rating (O), Country (N), Genre (N), Release Date (T), Runtime (Q)\end{tabular}                                      \\ \hline
\textbf{Popularity}         & \begin{tabular}[c]{@{}l@{}}Facebook Likes by Cast (Q), Facebook Likes by Lead Actor (Q),\\ Facebook Likes by Movie (Q), Popularity (Q)\end{tabular} \\ \hline
\end{tabular}
\caption{All attributes evaluated in our merged Movies dataset, grouped by attribute category. Data types are specified in parentheses: \textbf{Q}uantitative, \textbf{O}rdinal, \textbf{N}ominal, or \textbf{T}emporal.}
\label{tab:attributes} 
\Description{There are four attribute categories: ratings, finances, details, and popularity. Ratings includes the IMDB Vote Average (Q) and the IMDB Vote Count (Q). Finances includes Budget (Q), DOmestic Gross (Q), Profit (Q), and Worldwide Gross (Q). Details includes MPAA Rating ()), Country (N), Genre (N), Release Date (T), and Runtime (Q). Popularity includes Facebook Likes by Cast (Q), Facebook Likes by Lead Actor (Q), Facebook Likes by Movie (Q), and Popularity (Q).}
\vspace{-5mm}
\end{table*}
% To better understand the existing preferences participants have and how it impacts their decision-making, as well as the impact of analysis experience on user preferences,
% To address our research questions, 
We designed \highlight{an} online experiment to explore the relationships between visualization recommendations, user preference and trust. \footnote{Our research questions and exploratory hypotheses were pre-registered before running the experiment, available at \url{https://aspredicted.org/blind.php?x=tu5jk3}} In this section, we detail the design of our experiment, as well its limitations and trade-offs.



\subsection{Participants}
\label{sec:experiment-design:participants}

We recruited 114 participants via \url{Prolific.ac}, a crowdsourcing platform comparable to Amazon Mechanical Turk~\cite{peer2017beyond}. They were compensated \$3.35 for completing the experiment with an estimated completion time of 20 minutes, resulting in a projected \$10.05 hourly wage (and actual average wage of \$12.57 per hour). 

Recruited participants were at least 18 years of age with baseline data analysis experience (e.g., having taken a data science course, or worked in analytics). We chose to not impose more restrictive filters on experience to allow for a more diverse participant pool.
77\% of our participants identified as female. 80.5\% of participants were 18-24 years of age. 66.4\% had at least some college education.  

\vspace{-0.5mm}
\subsection{Experiment Dataset}
\label{sec:experiment-design:dataset}


In keeping with our broad recruitment criteria, we used movies as the basis for our experimental task because it is a domain with which the general public is somewhat familiar, and has extensive publicly available data.
We pooled attributes from three  movies datasets from Kaggle \cite{kaggle1,kaggle2,kaggle3} and the-numbers.com \cite{thenumbers} to provide a diversity of data attributes to explore. Certain attributes were omitted from our analysis for the following reasons:
\begin{itemize}[nosep]
    \item the attribute was redundant with another, already selected attribute
    \item the distribution of values was highly skewed (e.g., language)
    \item the attribute caused excessive visual clutter due to high cardinality (e.g., title, director)
    \item the attribute contained multiple values per tuple
\end{itemize}

The attributes list (\autoref{tab:attributes}) was provided to participants to give them an idea and explanation of what attributes could be explored, and was later used to create visualization recommendations.

The dataset was cleaned to prevent visualizations from having significant occlusion, extreme outliers, or other distracting artifacts. First, we sampled 200 tuples. Then for each visualization, we filtered out any outliers (i.e., tuples outside of the interquartile range) for each attribute rendered in the visualization. As our study examines the relevance of a visualization in terms of attributes, bivariate visualizations were generated that employ standard best practices for attribute encodings. Quantitative and temporal data is encoded using position, and categorical data with length \cite{mackinlay2007show}.

%We primarily focused on creating visualizations based on 11 quantitative variables (including profit, budget, and popularity) and 4 categorical variables (including MPAA-rating and genre) to ensure diversity of visualization types created. 
%\begin{itemize}
%    \item https://www.kaggle.com/carolzhangdc/imdb-5000-movie-dataset#movie\_metadata.csv
%    \item https://www.the-numbers.com/box-office-records/worldwide/all-movies/cumulative/all-time
%    \item https://www.kaggle.com/rounakbanik/the-movies-dataset#movies_metadata.csv
%    %this link contains an explanation of some of the features from the above Kaggle link
%    \item https://www.kaggle.com/rounakbanik/the-story-of-film
%\end{itemize}

\subsection{Experiment Overview}
\label{sec:experiment-design:overview}

\begin{figure*}[tb]
\centering
\includegraphics[width=0.7\textwidth]{figures/vis-bias-panels.png}
\caption{A snapshot of two visualization recommendation panels from the experiment interface. Each panel is labeled as either ``Human-Curated'' or ``Algorithmically-Generated,'' and assigned a random order position (left/right) and color (orange/blue). Color was used to further distinguish the recommendation source.} 
\label{fig:panels-example}
\Description{2 panels of 6 visualizations each are placed side by side, with the human curated panel on the left, and algorithmically curated panel on the right. Each panel is comprised of bivariate graphs, and are either bar graphs, scatter plots, or line graphs.}
\end{figure*}

%Our experiment was implemented as a single Qualtrics survey. All study materials are available at \url{https://osf.io/zmnh3/?view\_only=c3a9a1568d554c3587132b339c72f22e}.

Participants were given time to review and complete the consent form before beginning the study, and could withdraw at any point. Participants took 17 minutes on average (s.d. 9 minutes) to complete the survey. Those that were 3 standard deviations below the average time were to be excluded from our analysis, though none fell into this category.

We then gave participants the following scenario: ``a well-known film studio is hosting a competition for new movie ideas, and you are currently gathering information in preparation for a pitch on why your movie would be successful. To help you extract insights about successful movies, the studio has provided you with various metrics about movies that have been created in the past.''



% Participants were asked to consider a (fictitious) scenario where they are preparing to participate in a movie pitch competition being held by a major movie studio. They are analyzing movie data provided by the studio prior to writing their movie pitch.

Our study progressed in three phases, where participants:
\begin{itemize}[nosep]
    \itemsep0em
    \item \textbf{Phase 1}: record recommendation source preferences and attribute preferences for a given movies dataset;
    \item \textbf{Phase 2}:  rate two separate groups (or panels) of visualization recommendations, and select one panel to proceed with; and
    \item \textbf{Phase 3}:  complete surveys collecting experiences with the recommendation panels and demographic information.
\end{itemize}
%In the first phase, we solicited participant's prior preferences for algorithmic versus human decision-making, and then solicited a ranked list of data attributes (i.e., columns) present in our movie dataset. In phase two, participants were presented with a panel of ``Human-Curated'' recommendations and a panel of ``Algorithmically-Generated'' recommendations, and had to select one panel for further analysis (see \autoref{fig:panels-example} for examples). In reality, the assignment of these panel labels was random: all panels were hand-generated, and represented a range of relevance scores with respect to important attributes in the data, which we derived from informal pilot studies. We then recorded participant's preferences for one panel over the other. In phase three, we solicited free-text responses justifying their reasoning.
A pilot study of 12 participants was run prior to our main study to test our materials and procedure. 

\subsection{Phase 1: Recording Prior Preferences}
% \highlight{\sout{To understand how participants choose between recommendations, we first need to understand their prior interests and biases.}} 
We \highlight{captured} participants' priors in two ways: by asking participants to rank the movies attributes they \highlight{were} most interested in analyzing, and by asking participants about their general prior preferences for human-curated versus algorithm-generated recommendations.

\subsubsection{Ranking Attributes of Interest}
%The experiment was largely formulated around a central task posed to participants. 

Before seeing any visualization recommendations, participants were provided a list of all data attributes (with corresponding explanations) present in the movies dataset, and asked to rank the top five attributes they would like to reference while creating their pitch.

This ranking task helped participants to familiarize themselves with the available attributes for analysis, and helped us to gain an initial understanding of the attributes participants wanted to see in later visualization recommendation panels. While these rankings were not used to generate visualizations, they helped us assess the expected relevance and utility of the panels that were displayed to participants in the later stages of the experiment.
%This was done to familiarize participants with the features of the movies dataset, and to engage a more analytic mindset.
%It also served as an important way for us to evaluate the efficacy of our relevance metric, by evaluating whether the panels were generated from attributes participants actually found to be helpful.

\subsubsection{Soliciting Prior Recommendation Preferences} 
We then asked participants whether they prefer recommendations from humans, algorithms, or neither (i.e., no preference), in the context of song recommendations. Though song recommendations may not fully generalize to the context of visualization recommendations, we aimed to capture prior preferences in a familiar context where many people encounter both automated (e.g., Spotify mixes~\cite{spotify}) and human recommendations (e.g., personally curated playlists). This mixture of familiarity and transferability was useful for the task without narrowing the participant pool to those with direct experience with visualization recommendation systems.

%chose a familiar domain to avoid narrowing our participant pool to those with direct experience with visualization recommendations. A separate domain also helps to prevent priming effects.
% Participants were then asked for their human versus algorithmic preference in the context of song recommendations. The song recommendation context was specifically chosen to prevent  priming effects while still being a familiar domain for most users. This helped to establish a baseline of prior preference. 
%By soliciting prior recommendation preferences, we have a ground truth baseline to compare with participants' selected visualization recommendation panels later in the experiment.

\subsection{Phase 2: Comparing Recommendation Panels}
\label{sec:experiment-design:comparing}

Once the participant's initial preferences were recorded, the participant was then asked to compare two separate panels of visualizations (see \autoref{fig:panels-example} for example panels).  These panels are comprised of 6 visualizations of 3 possible types: line chart, bar chart, or scatterplot. Our focus on panels over individual charts is motivated by the design of existing recommendation systems (e.g.,~\cite{wongsuphasawat2015voyager, mackinlay2007show, vartak2015s}) which present multiple visualization recommendations at a time. One panel was labeled  as ``Human-Curated'' and the other as ``Algorithmically-Generated.'' However, both were in fact generated by the authors and these labels were assigned randomly.

Participants were asked to rate how useful each panel would be for completing the task (analyzing data to support a movie pitch) on a ten point Likert scale, and to select a single panel for their analysis. After making a selection, participants were asked to explain their choice of panel. The ratings and final selection enabled us to gather information on the perceived relevance of each panel.
%, and to later evaluate the potential impacts of ordering and coloring. Ultimately, participants were asked choose either a “Human-Curated” recommendation panel or a “Algorithmically-Generated” to use in developing their pitch and asked to explain their reasoning behind the choice. This response would later come to form the bulk of our qualitative analysis, by providing insight into a user's decision-making process.

%not sure how necessary the below paragraph is but leaving it in here for now
% After seeing the visualizations, participants were also given the opportunity to re-rank their top five attributes. This re-ranking option allows us to gauge whether the initial top five ranking results are a reasonable approximation of participants' interests or not. For example, if few participants change their rankings after seeing the recommendations, then the original rankings are likely to be a reliable guide for a participant's interest in the dataset.
 
 After a specific recommendation panel was selected (either human or algorithm), the participant was asked to describe what they learned from this panel that would help them in writing a movie pitch. The participant was then asked to rate the panel based on how helpful it was in forming insights based on a 10 point Likert scale, and asked if there was anything they would have liked to see as part of the recommendations.

\subsection{Phase 3: Completing Final Surveys}
The final phase of the experiment involved completing two surveys for capturing participants' decision-making processes and overall impressions, as well as demographic information.

First, participants were asked a series of 8 questions asking the extent to which participants agreed to various statements about the quality of human recommendations and algorithm recommendations, and any perceived differences between the two recommendation sources.
For example, participants indicated their agreement with such statements as ``The algorithm did a good job in selecting the visualizations that I should analyze,'' ``I felt that key visualizations were often missing from the recommendations,'' and ``There was a noticeable difference in the quality of recommendations between humans and algorithms'' on a 5 point Likert scale. The survey concluded with demographic questions, including collecting gender, age, and educational attainment to prevent priming. 
%This was done to better understand the participant's own evaluations of the recommendations, and would not only provide insight into their decision-making process, but would help understand whether our relevance metrics matched their perception of relevance.

\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{figures/scoring_example.pdf}
    \caption{A demonstration of how visualization recommendation panels are scored, with four visualizations taken from \autoref{fig:panels-example} as examples. Higher ranking attributes award more points than lower-ranking attributes, and the narrow dynamic range of high-impact panels causes us to remap all panels with particularly high scores.}
    \Description{Examples of how to calculate visualization panel relevance scores based on 5 attributes (budget with a weight of 5, popularity with a weight of 4, MPAA Rating with 3, Genre with 2, and Profit with 1). 2 example panels are displayed. Panel A has a score of 10, because one visualization has a score of 6 and the other score a 4. These visualizations got their scores because one visualized MPAA Rating (3) with profit (1), which sums to 4. Similarly, the other visualization was budget(5) and Genre (2) which sums to 7. All ratings greater than 6 get mapped to 6.}
    \label{fig:scoring-example}
\end{figure*}
\vspace{-0.3mm}
\subsection{Computing Recommendation Panel Relevance}
To better understand how participants’ panel selections may be influenced by prior preferences, we designed four panels of varying relevance. In this way, we could see whether participants’ panel selections were in alignment with the perceived relevance of the panels (i.e., in alignment with their top five attributes of interest). 
% Here, we explain our process for constructing these panels.

\label{sec:experiment-design:relevance}

\subsubsection{Scoring Individual Visualizations}
Before scoring the quality of entire panels, we first created a method to score individual visualizations.
%To first create the panels of visualizations, we had to select features that participants would find to be helpful. As part of our experiment, we ask participants to select 5 attributes they find to be the most useful in subsequent analysis.
We had performed an initial pilot study with 12 participants, where we created panels from 5 randomly selected attributes but otherwise followed the current study design. Through that pilot, we found that the top five most popular data attributes were (in order of frequency): budget, popularity, MPAA rating, genre, and profit (also shown in \autoref{fig:scoring-example}).
These attributes served as the basis for constructing high and low relevance visualization recommendations.
We applied a simple linear weighting system to assign a weight to each of these attributes (budget received a weight of five, popularity a weight of four, and so on). All other attributes were assigned a weight of zero. Though other weighting mechanisms, such as exponential or quadratic, could have been used, as participants were ranking them in a linear fashion, we felt it prudent to use a linear weighting to match. 

At first, a single visualization ranged from a score of 0--9. As only a few visualizations could have a score of 6--9, we clamped all scores higher than 6. The resulting 0--6 per-visualization scoring lends itself to a more even distribution. Relevance for the bivariate visualization was calculated by summing the weights of the two corresponding attributes.
For example, consider the first visualization in example panel A of \autoref{fig:scoring-example}, which visualizes MPAA Rating versus Profit. MPAA Rating has a weight of 3, and Profit a weight of 1, producing a summed score of 4. In contrast, the first visualization of example panel B has no relevant attributes, producing a relevance score of 0.

%For example, a visualization showing profit vs. genre would have a score of 3. Notably, there were only a few visualizations that could have a score of 6, 7, 8, or 9. In order to create a more even distribution of scores, we decided to bin visualizations in the range of 6-9 and reassign them to a value of 6. We grouped relevant visualizations into three categories based on their score: 
%
%	least relevant: score of 1-2
%	relevant: score of 3-4
%	most relevant: score of 5-6
%
%This scheme provided a consistent way to evaluate the relevance of an individual visualization based on its component encodings.

\subsubsection{Panel Generation Strategy}
\label{sec:experiment-design:panel-generation}
Using the scoring mechanism for individual visualizations, we then computed scores for entire recommendation panels. For example, to calculate the final scores for example panels A and B in \autoref{fig:scoring-example}, we sum the corresponding visualizations, producing combined scores of ten and one, respectively.
Note however that each panel from our study consists of six separate visualization recommendations.
%Then, we needed a way to determine the relevance of an entire panel of visualizations.
Three of these visualizations were chosen to be relevant (i.e., with a score greater than zero), and the rest were selected to be irrelevant (i.e., have a score of zero).
%Panels comprised of 3 visualizations with a score greater than 0, implying a degree of relevance, and 3 visualizations with a score of 0, meaning that they do not contain a ranked attribute. To determine the thresholds of relevance for a composite set of visualizations, we analyzed the distribution of panel scores by computing all possible ways to pick 3 relevant visualizations. For example, picking three visualizations from the “most relevant” visualization category results in a grid with a score of 15-18, by summing up the scores of the component visualizations. Picking two visualizations from the “relevant” category and one from “less relevant” results in a grid with a score of 7-10. Similar to the visualization scoring, we grouped grids into three categories based on their score:
%
%	least relevant: score of 3-8
%	relevant: score of 9-12
%	most relevant: score of 13-18
%
%Thus, we had a way of empirically assessing the relevance of a panel by its component visualization scores. The resulting 2 "High Relevance" panels and 2 "Low Relevance" panels were integrated into the experiment.
With possible panel scores ranging from 3--18, to compute two ``high relevance'' panels, we generated two recommendation panels with scores in the range of 13--18. To compute two ``low relevance'' panels, we generated two panels with scores in the range of 3--8. For example, panel A from \autoref{fig:scoring-example} could be the starting point for building a ``high-relevance'' panel, and panel B a ``low-relevance'' one. Panels were also chosen to have at most one repeating data attribute to ensure a breadth of visualized attributes.

\subsubsection{Permuting Panel Pairings}
\label{sec:experiment-design:pairings}

Given our two ``high relevance'' panels and two ``low relevance'' panels, we have six total pairing scenarios: high-high (one pairing), high-low (four pairings), and low-low (one pairing). Taking panel order into account, we have 12 possible ordered pairs for comparison. Each ordered pair represents a separate condition of our experiment. Color and ordering of human versus algorithm labels were controlled by randomizing across participants. We collected data until at least eight participants completed each of our 12 experiment conditions.

%\subsection{Experimental Conditions}
%We test 12 conditions based on the permutation of relevant and irrelevant panels. There were 2 different high-relevance panels and 2 low-relevance panels, forming 4 * 3 = 12 different permutations of grid arrangement. Color and ordering were randomized to prevent the biasing effect of order or aesthetics. 2 panels of highly relevant visualizations and 2 panels of low relevance visualizations were randomly paired into 12 sets of grids, which formed the condition groups that participants were randomly assigned into. 



\subsection{Experiment Design Limitations \& Trade-offs}
\label{sec:experiment-design:limitations}

\begin{figure*}[htbp]
\centering
\begin{minipage}{0.9\columnwidth}
  \centering
\includegraphics[width=\textwidth]{figures/test2.png}
\subcaption[first caption.]{A distribution of panel rating by number of common \\ features, or attribute overlap.}
\Description{A histogram of total attribute overlap. The histogram has a slight right skew, with most participants having at least 3 attributes overlap.}
\end{minipage}%
~%
\begin{minipage}{0.9\columnwidth}
  \centering
\includegraphics[width=\textwidth]{figures/panel_id_ratings.pdf}
\subcaption[second caption.]{A distribution of relevances by panel ID, calculated with a 95\% confidence interval and 1000 bootstrapped iterations. HR refers to a high relevance panel, and LR refers to a low relevance panel.}
\Description{A swarm plot visualizing the distribution of relevance scores by panel ID (HR1, HR2, LR1, and LR2). Participants rated all panels similarly, with ratings around 6 out of 10.}
\label{fig:1b}
\end{minipage}%

\caption{Participants rated all panels as similar in relevance, regardless of number of relevant features included in the panel }\label{fig:figure1}
\end{figure*}


To design our experiment, we had to consider multiple trade-offs, which we discuss here.

\textbf{All panels were human-curated}:
Human-curated and algorithmically generated recommendations are likely to be qualitatively different. Our decision to make the panels identical, but changing only the purported source, allows us to isolate the impact of source alone, but does not capture these potential visual and semantic differences.

\textbf{Fixed Panels and Relevance}:
Four panels were computed in advance, based on a fixed set of attributes collected from our pilot study. Features such as visual encoding, information density, and attribute pairing were uniform across these panels, as we chose to vary only attribute relevance across these panels. While we considered tailoring panels based on participants' rankings, as well as varying the visual encodings, the strength of this design is that it keeps the number of experiment conditions at a manageable level. 
% However, the true relevance of a panel with respect to a specific participant may not be the same as our a priori relevance score. As part of our analysis in \autoref{sec:analysis}, we evaluate differences between our a priori relevance and the ``true'' relevance of panels per participant.
However, we acknowledge that attribute relevance is only one dimension of visualization quality, and that visual encodings and interaction effects of attribute pairings were not accounted for. We chose a simple relevance metric as a starting point rather than a more complex reactive measure or stimuli generation procedure. 

\textbf{Single Trial Design}:
In our experiment, a single trial consists of participants evaluating one pair of panels. While one recorded preference per participant limits statistical power, it also avoids bias from multiple explorations of the same dataset. It also allows the experiment to be easily crowdsourced to a platform like Prolific.

\textbf{Wide Range in Participant Expertise}:
By not constraining participation by experience, our user population may not accurately reflect the population that commonly use visualization recommendation features. Though another study with a different population would help generalize the results, this design allows us to directly observe how data analysis experience influences user recommendation preferences.

\textbf{Using Color to Distinguish Algorithm and Human Panels}:
Though color was randomly assigned as a way to distinguish between recommendation source, a small number of participants used it as a basis for their decision. In consideration of this subgroup, other means of distinguishing between algorithm versus human could have been used. 

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/discussion.tex <==
\section{Discussion}

From our quantitative and qualitative observations, we synthesize the following preliminary findings: 

\textbf{People seemed to choose panels by focusing on the information presented in the visualizations.} In examining the rationale behind panel choices we found that, for a majority of participants, their decision-making process often focuses on the relevance of the data itself. We found some evidence that that \emph{people may rate recommendation panels based on the level of attribute overlap}. For example, participants may emphasize the cumulative information gained from a panel. We refer to these participants as \textit{all-rounders}, as they seem to obtain value from the quantity of information in a panel. However, some participants rely on a particular visualization as a deciding factor, indicating that prior preferences (and therefore biases) may still play a role in subsequent decision-making. We refer to this cohort as \textit{seekers}, as they seem to be looking for a specific chart or set of charts to investigate specific hypotheses.

Our results point to the existence of differing patterns of information foraging among viewers, suggesting that there may not be a one-size-fits-all solution to the problem of recommending useful visualizations. To better support these different user groups, we suggest tailoring recommendations towards different patterns of analyses. For instance, recommendations for all-rounders could focus on presenting dashboards that present overviews of many key metrics, whereas recommendations for seekers could focus on specific attributes of interest or particularly informative visualizations (in the information-theory sense~\cite{chen2010information}). These suggestions might require the collection of priors or other data-driven inference about data, rather than just the surfacing of arbitrary ``data facts''~\cite{srinivasan2018augmenting} such as outliers or strong correlations. 


%Likewise, a fifth of participants reported that the source of recommendations was important to them, suggesting a need for explainable and transparent recommendations. \textbf{I trust it but I don't know why -- users relying on other features / gut instincts it's hard to distinguish between various options}


%Explanations could potentially increase trust and reduce bias regardless of the participants’ source preferences. 


%RQ1
\textbf{Existing preferences are not predictive of subsequent recommendation choice, though perceptions of source can contribute.} While participants initially
% \highlight{\sout{generally}} 
preferred human recommendations, their subsequent panel choices revealed an insensitivity to recommendation source. Similarly, Peck et al. found that over half of participants did not change their initial rankings of the usefulness of visualizations after the sources (e.g., government agencies, universities) of each visualization were revealed~\cite{peck2019data}. That said, around a fifth of participants in our study indicated that the source of recommendations was important to them, and some perceived differences in the reliability and accuracy of human and algorithmic recommendations.  

% \highlight{\sout{Additionally,}}
Designers should consider how to present information in an unbiased manner for these individuals with clear preferences for recommendation source. For example, visualization recommendation systems might provide more detailed information on how the recommendations were curated to help users develop more trust in the system as a whole ~\cite{YangVisualExplanations}. However, more research is needed to determine an appropriate threshold for transparency: providing too much or too little transparency can erode trust in algorithmic recommendations~\cite{Kizilcec2016}.  


%This supports our second hypothesis, that an \emph{a priori preference for human versus algorithmic recommendations largely did not bias participants towards a particular panel}. However, 
%We also found that 14\% of participants adhered to their existing preference despite the lower relevance of the associated panel. 


%RQ3



%These user populations should be considered carefully when designing new visualization recommendation features, .
%, as the barrier to sophisticated visualization software lowers.

%RQ2

\textbf{Data analysis experience does not have a substantial impact on preferences or panel selections, although visualization comprehension and aesthetics may play a role}. Challenges in understanding certain visualizations (e.g., scatterplots) may have hindered some participants' ability to effectively evaluate recommendations. Although a recommendation panel may have useful information, it is only relevant if the user can meaningfully interpret its data. Future work may solicit more information about participants' personal backgrounds to gain deeper insight into factors that influence people's perceptions of relevance beyond data analysis experience. While analysis experience did not seem to impact participants' panel selections, aesthetics shaped a minority of participants' decisions. As the audience of visualization tools broadens over time, designers should consider the aesthetics of visualizations as a means of supporting users' understanding of the data and encouraging them to interact with the system \cite{moere2011role}.

%Both our quantitative and qualitative results suggest that people, in our decision task, are willing to be flexible in their assessment of visualization recommendations, regardless of their initial beliefs about the source of these recommendations, and make decisions based on their anticipated data-related needs.

%In assessing the basis of our analysis, the relevance metrics, We find that our fixed rankings and fixed relevance scores seem to align with participants' attribute rankings and adjusted relevance scores. 
% To evaluate whether participants actually perceive our high-relevance panels as being more relevant compared to the low-relevance panels, we analyze participants' panel ratings. 
%We find that the \emph{relative difference} in ratings for a given pair of panels appears to matter more than the actual ratings themselves. Taken all together, these findings seem to suggest that \textbf{our fixed relevance scoring mechanism is in alignment with participants' perceptions of panel relevance.}

%Furthermore, we find that participants seem to ascribe higher ratings to and ultimately select recommendation panels that overlap more with their attribute ratings. Thus, our results seem to suggest that \textbf{participants prioritize visualization recommendations by attribute relevance}, supporting hypothesis \textbf{H1}.

%Afterwards, we delve into participant preferences, and find that participants begin the experiment with a modest preference for human-curated recommendations. However, as participants evaluate recommendations and choose between panels, we find that this initial bias effectively disappears. These findings also appear to be consistent with our previous relevance analysis: participants generally seem to ascribe higher ratings to and select panels that are more relevant, where in our experiment design, relevance is independent of recommendation source.

%Though far from the majority, we do find that a notable fraction of participants stick with their preferred recommendation source, even when it turns out that the corresponding panel is less relevant, partially supporting hypothesis \textbf{H2}.

Overall, our results are positive news for the designers of visualization recommendation systems. Neither of the failure cases we mention in this paper, either the uncritical acceptance of recommendations from algorithmic sources, nor the knee-jerk rejection of the same, appear to occur with high frequency. However, we note that this pattern of apparent rationality is not universal: a sizable portion of our adherents stuck with their preferred choice of recommendation source even given measurable mismatches in expected utility. This behavior suggests that we either lack appropriate measures to assess the utility of visualization recommendations, or that users rely on additional factors to evaluate perceived differences between recommenders. As a consequence, future work may investigate the qualitative and quantitative differences between human and algorithmic data visualizations to identify specific factors influencing trust. The presence of these adherents, combined with a substantial initial preference for human recommendations, also suggests that there is value (and some risk) in providing human recommendations, which may be perceived as having intrinsic authority and relevance over algorithmic choices. 
% Even more troubling, confirmation bias appears to be at play. Despite the relative uniformity in utility in chosen versus non-chosen visualization panels, people still rated their own choices as being more useful. 


% Our study presented a limited set of recommendations about an abstract task, and solicited feedback in a holistic way. The reasons why people may prefer one visualization over another may be complex and multifaceted, and highly dependent on a specific task. We acknowledge that we chose a simple relevance metric as a starting point rather than a more complex reactive measure, and that we solicited prior preferences based on a single task-irrelevant domain. Future work may explore more exhaustive measures to solicit prior preferences and judge the true relevance of recommended visualizations. 

% We also note that the deceptive nature of our experiment and the use of randomized labels means that there was no a priori expected gain or loss in utility for preferring one source over the other. In reality, algorithmic recommendation systems may have performance that characteristically diverges from human recommendations. Future work might evaluate systematic differences in the recommendations that humans and algorithms create. 
%Furthermore, algorithmic performance might only be detectable over repeated sessions of analysis. The long-term building (or degrading) of trust remains outside of the scope of our current experimental design. 

% Additionally, our test population may not be representative. Most participants were between 18-24 years of age and had at least some college education. Another study with a different population would be needed to generalize the results.

% Lastly, our study was exploratory in nature: we did not feel that existing measures for trust or visualization recommendation quality were mature enough to directly apply to our cases of interest in ways that would support direct statistical modelling or inferential tests. It remains to future work to scope, expand, and validate existing measures for these experimental tasks.


==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/introduction.tex <==
\maketitle
\section{Introduction}
\label{sec:introduction}

% As a field and an industry, visual analytics is beginning to incorporate increasingly automated methods into its processes~\cite{heer2019agency}. These automated methods are often used to create visualization \textit{recommendations}. 

As a field and industry, visual analytics is beginning to incorporate increasingly automated methods into its processes~\cite{heer2019agency}, often to create visualization recommendations. From academia, visualization systems like Draco~\cite{moritz2018formalizing}, Data2Vis~\cite{dibia2018data2vis}, and Tableau's Show Me Feature~\cite{mackinlay2007show} attempt to automatically generate expressive and informative visualizations from a dataset. In industry, features like PowerBI's ``Quick Insights'' panel~\cite{powerbi} attempt to present quick visual summaries of interesting or important aspects of a dataset. 

% In contrast to these automatic methods, much of the work of summarizing, selecting, and designing visualizations is done manually. Data summaries like dashboards are often designed with deep thought and intensive manual labor for the use cases and intended audiences of the data~\cite{sarikaya2018we}.

While the relative trustworthiness of machine learning models has been investigated in other contexts~\cite{castelo2019let,jakesch2019ai,Yin2019accuracytrust} there has been little investigation of viewers' trust of recommendations in visual analytics. Though widely used visualization authoring software like Tableau and PowerBI incorporate recommendations, users may adopt the authoring portion of the tool without trusting or utilizing the recommendation features; many recommendation systems in popular tools such as ``Explain Data'' in Tableau \cite{tableauexplain} are relatively new, with unclear adoption. If analysts are wholly trusting of algorithmic recommendations, potentially biased or inaccurate results could result in poor decision-making \cite{correllEthical}. However, if analysts habitually devalue automated insights or recommendations, existing research efforts into automated visualization recommendations may be misaligned with their needs. 

In this paper, we present the results of a pre-registered, exploratory human-subjects study on how the perceived source (human or algorithmic) of visualization recommendations impacts assessments of the utility of those recommendations for general audiences. We sought to determine if existing attitudes and biases regarding algorithmic recommendations on the whole would impact people’s assessments of the quality of visualization recommendations, and whether these biases would persist even as we adjusted the anticipated relevance of the recommendations.

%In this paper, we present the results of a pre-registered, exploratory human-subjects study on trust in visualization recommendations in general audiences. 
% Our study design was informed by the designs of existing visualization recommendation systems in industry and academia
%, such as Tableau's Show Me feature~\cite{mackinlay2007show} and the Voyager system~\cite{wongsuphasawat2015voyager,wongsuphasawat2017voyager}.
%We sought to determine if existing attitudes and biases regarding algorithmic recommendations would impact people's assessments of the quality of visualization recommendations, and whether these biases would persist even as the utility of particular recommendations changed.

Through a quantitative and qualitative analysis of our collected data \footnote{Our study materials, including data tables and analyses scripts, are available at \url{https://osf.io/zmnh3/?view\_only=c3a9a1568d554c3587132b339c72f22e}},
%we found that, while many people have their own preconceptions on the utility of algorithmic versus human-curated visualization recommendations, these prior beliefs seem less relevant than the human's own assessment of the utility of the recommendations, pointing to a flexibility in attitudes towards recommendation systems largely agnostic of their source. Specifically, 
we found that participants initially preferred human-curated recommendations, but tended to be source-agnostic when evaluating visualization recommendations of equal quality. This appeared to hold even across different levels of analytics experience. Participants' evaluations of recommendation sources seemed to emphasize the degree of overlap between the participant's top attributes of interest and the attributes displayed in the recommendations. In stating their rationale for preferring one set of recommendations over another, participants fell into two categories of behavior: \emph{all-rounders} tended to focus on the quality of recommendations as a whole, while \emph{seekers} honed in on the presence of particular visualizations or attributes.
% Participants' stated rationale for preferring one set of recommendations over another focused on either the quality of recommendations as a whole, or the presence of particular visualizations or attributes.
% Nevertheless, we found a  fraction of participants who stuck with their a priori source preference, even when this source presented recommendations we measured as being less relevant  (14\%), suggesting a confirmation bias amongst these participants.

Our findings partially support existing assumptions in the community that users trust automated visualization recommendation systems. Though some participants held onto folk theories about the capabilities of a given recommendation source, users on the whole exhibited different mental models on evaluating the utility of recommendation panels. These observations suggest that users are not uniform in how they evaluate, and subsequently determine the utility of, visualization recommendations.
% Our results point to the existence of differing patterns of information foraging among viewers, suggesting that there may not be a one-size-fits-all solution to the problem of recommending useful visualizations.
We reflect on how designers can present recommendations to a broad range of users in a way that mitigates the risk of user bias in interpreting the results, contributing to an emerging body of work on algorithmic trust.

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/motivation.tex <==
\section{Motivation and Research Questions}
\label{sec:motivation}
When we compare the literature on user trust in algorithmic decision-making to that of visualization recommendations, we find a contradiction: visualization recommendation features are designed as if users will naturally trust them, yet in other contexts users express a clear distrust of algorithmic decision-making. To the best of our knowledge, no existing studies explicitly measure user trust in algorithm-generated (versus human-curated) visualization recommendations. 

% These competing (and missing) perspectives serve as the core motivation for our work:
The absence of research on the perceived trustworthiness of existing recommendation systems, as well as the potential mismatch between these systems and human mental models, serve as the core motivation for our work:
if the user is biased against recommenders, then expending resources on generating recommendations may prove wasteful, but if the user blindly trusts all recommendations (including occasional bad ones), the user may inadvertently draw inaccurate (and potentially dangerous~\cite{bresciani2015pitfalls}) conclusions. 
%%by ignoring whether the user even trusts system-generated visualization recommendations in the first place, we may be wasting valuable time and resources producing recommendations that the user will ultimately ignore.
In this work, we seek to explore the following research question: 

\noindent\textbf{Research Question 1}: \emph{How do existing preferences for human-curated versus algorithmically-generated recommendations affect the evaluation of recommendation quality or utility?}

Specifically, we seek to understand whether the source of recommendations (human or algorithmic) may alter a user's perception of the recommended charts. Obtaining a deeper understanding of why users prefer certain recommendations over others can help visualization system designers to better employ techniques to support a wide range of users. To further understand the context for user preferences, we explore the following secondary analysis questions:

\noindent\textbf{Research Question 2}: \emph{If clear preferences are observed, what reasons do users give for preferring certain recommenders?}

%That is, can we attribute these preferences to judgments about the \textit{source} of the recommendations, the specific \textit{content}, or some combination of factors?

    %\item Do our visualization panel designs (i.e., relevance judgements) match the relevance judgements of the participants? Were our panels based on attributes that participants found to be important? 
\noindent\textbf{Research Question 3}: \emph{What effect (if any) does statistical or data analysis experience have on user preferences?}

% If we can determine whether users generally trust visualization recommendations, or detect which users will be more open to them, then we can help visualization system designers to better employ techniques to support a wide range of users.

%design more effective visualization systems to support these different users.
% Furthermore, with a deeper understanding of why users prefer certain recommendations over others, we can improve upon existing visualization recommendation strategies.
% To provide additional context for why users may express certain preferences, we seek to investigate the following secondary analysis questions:



    %\item Do people with more statistical or data analysis experience have different preferences than those with less experience?

\noindent\textbf{Exploratory Hypotheses}:
Based on the above research questions, and to capture our expectations for how user trust may (or may not) manifest in our study, we formulated two exploratory hypotheses:

\begin{itemize}[nosep]
    \item \textit{People will rate recommenders based on how much the recommendations overlap with preferred data attributes.} 
    % That is, that people will assess the relevance and utility of recommendations in based on their contents.
    \item \textit{Prior preferences for human or algorithmic recommendations will bias participants towards the corresponding panel, even in the face of differing amounts of recommendation relevance.} 
    % That is, that existing preferences or biases may shift assessments based on the perceived source of the recommendations, regardless of their assessed utility.
\end{itemize}

==> [CHI 2021] Vis Bias (DOUBLE COLUMN)/content/related_work.tex <==
\section{Related Work}
\label{sec:related-work}
Our research questions and experiment design are informed by existing assumptions for visualization recommendation systems, as well as studies measuring users’ preferences for algorithmically generated recommendations in other contexts. We highlight three topics of related research: visualization recommendation systems, inclusion of contextual information, and trust in algorithmic decision making.

\subsection{Visualization Recommendations}
\label{sec:related-work:recommendations}
A number of systems recommend sets of visualizations based on various assumptions (or explicit solicitation) of information and patterns that users would find valuable. Golfarelli et al.~\cite{golfarelli2019model} propose a pipeline for generating visualization recommendations based on a set of \highlight{predefined} user objectives. Wongsuphasawat et al.~\cite{wongsuphasawat2015voyager,wongsuphasawat2017voyager} provide flexibility by allowing users to specify partial visualization designs, and recommend visualizations that extend these partial specifications. 
Vartak et al. identify statistically significant differences between sub-populations within a dataset, and recommend bar charts capturing these differences~\cite{vartak2015s}. 

The number of recommendations vary per system as well, which impacted our experimental design. Some systems, such as Calliope~\cite{calliope_2020} and ``Retrieve Then Adapt''~\cite{retrievethenadapt}, focus on recommending a single visualization, such as a data story or infographic. In most cases, users are provided an ensemble of recommendations grouped together in a single \emph{panel}. Voyager is a salient example, and so we adopted a similar design for our study~\cite{wongsuphasawat2015voyager,wongsuphasawat2017voyager}.
% Hu et al.~\cite{hu2019vizml} and Dibia and Demiralp~\cite{dibia2019data2vis} train machine learning models on massive visualization corpora to recommend visualization designs for new datasets. 

% Moritz et al. treat visualization design knowledge and best practices as constraints on the visualization design space, and implement a pipeline for generating recommendations given a concrete set of design constraints~\cite{moritz2018formalizing}.
% Srinivasan et al. extend these recommendation ideas by generating interactive facts about a given dataset to augment visual analyses~\cite{srinivasan2018augmenting}.  
Though these systems employ differing strategies, they appear to be developed under the implicit assumption that users generally want and trust algorithmically-generated visualization recommendations. Given that the differences between human and algorithmically-generated visualizations are not well understood, we shed light on user trust in recommendation source through the use of labelling, similar to Jakesch et al. and Shank et al. ~\cite{jakesch2019ai, shank2013computers}. That is, we present participants with visualizations that were all created by humans, but some were labelled otherwise.

% In this work, we shed light on whether people trust recommendations when they are told they are algorithmically generated versus human curated. The differences between human and algorithmically generated visualizations are not well quantifiable, so we instead only varying the labelling, inspired by Jakesch et al.~\cite{jakesch2019ai}'s work with Airbnb profiles.


% In this work, we shed light on whether people trust algorithmically generated visualization recommendations, and how preexisting preferences may impact the way users respond to them.

%\vspace{-3mm}
% \subsection{Bias in Visualization Preferences}
% \label{sec:related-work:bias-deception}

% Several projects have explored how perceptual and cognitive biases may impact the way people interpret and make decisions using visualizations.
% % Wall et al.~\cite{wall2017warning} propose an approach to detecting cognitive biases as users interact with visual analysis tools, and suggest strategies to relay this information to users.
% %Correll and Gleicher~\cite{correll2014error} observe that the way in which error is represented in visualizations (e.g., error bars, violin plots, etc.) could inadvertently lead users to interpret the data in a biased way.
% % Kim et al.~\cite{kim2017data} investigate whether observing the expectations of others may influence how individuals interpret visualizations, and find that people may become biased when their own expectations match those of others, even when these expectations are incongruent with the actual data. 
% %Similarly, Xiong et al.~\cite{xiong2019curse} show that preconceptions about interesting features in a dataset can result in the ``curse of knowledge'' when recommending features in the data to others.
% When visualizing personal informatics data, van Dijk et al.~\cite{van2016deceptive} observe that a user's expectations for how the data should look often alters (and ultimately biases) the user's perception of the visualizations.
% Dimara et al.~\cite{dimara2018task} survey the various empirical findings and viewpoints on cognitive bias in the literature, and organize them into a seven-category taxonomy for cognitive bias in visualization.
% Through semi-structured interviews with residents of rural Pennsylvania, Peck et al. explored the factors that inform attitudes and perceptions about data visualization. They found that participants relied heavily upon their personal experiences in the decision-making process (e.g., prioritizing graphs that are personally relatable) and valued clarity, simplicity, and visual appeal. \cite{peck2019data}

\subsection{Inclusion of Contextual Information}
\label{sec:related-work:metadata-pref}

Several projects have explored the potential ways in which additional contextual information impacts how people interpret and evaluate visualizations.

The ``Contestability in Algorithmic Systems'' Workshop at CSCW 2019 argues for the inclusion of humans in the loop of algorithmic decision making, especially as decisions made by machine learning systems have greater consequence. One of their design objectives to do so is through \textit{legibility}, in which systems would include explanations for the decisions made and conclusions drawn \cite{contestability}. 

There are many projects that explore legibility, especially in machine learning systems. Yang et al.~\cite{YangVisualExplanations} found that additional metadata, in the form of example-based explanations for machine-learning classifiers, did improve user trust, although Kizilcec~\cite{Kizilcec2016} \highlight{found that} that providing \textit{too much} explanatory information can erode trust. Cheng et al.~\cite{cheng2020dece} take this one step further and propose DECE, a visual interactive system to better understand the decision rules of machine learning systems through counterfactual explanations. 

However, these systems are focused on machine learning in particular. Peck et al. explore the notion of metadata, in this case the source of the data, in relation to perceptions of visualizations~\cite{peck2019data}. Through semi-structured interviews with residents of rural Pennsylvania, they \highlight{gathered} initial perceptions and rankings of visualizations without participants knowing the sources of visualizations. Afterwards, they \highlight{revealed} the sources and \highlight{asked} whether knowing the sources of the graphs impacted how participants viewed them, as well as their overall ranking. They found that 60\% of participants chose not to re-rank their visualizations after revealing the sources, indicating that for some, additional context about source may not impact the perceived utility or credibility of a visualization.



% Wall et al.~\cite{wall2017warning} propose an approach to detecting cognitive biases as users interact with visual analysis tools, and suggest strategies to relay this information to users.
%Correll and Gleicher~\cite{correll2014error} observe that the way in which error is represented in visualizations (e.g., error bars, violin plots, etc.) could inadvertently lead users to interpret the data in a biased way.
% Kim et al.~\cite{kim2017data} investigate whether observing the expectations of others may influence how individuals interpret visualizations, and find that people may become biased when their own expectations match those of others, even when these expectations are incongruent with the actual data. 
%Similarly, Xiong et al.~\cite{xiong2019curse} show that preconceptions about interesting features in a dataset can result in the ``curse of knowledge'' when recommending features in the data to others.




% User bias can potentially be exploited by visualization authors (and systems) to lead users to draw conclusions that may not accurately reflect the underlying data~\cite{correll2017black}. Several projects investigate how deceptive visualization design tactics could be applied to mislead users.
%Correll et al.~\cite{correll2018looks} observe that suboptimal settings for seemingly subtle visualization parameters, such as opacity and histogram bin size, can inadvertently (or in adversarial contexts, intentionally) hide important features and errors within data distributions.
% Pandey et al.~\cite{pandey2015deceptive} evaluate the effectiveness of common visual distortions as deceptive tactics to manipulate users through visualization design, and find these techniques are actually effective in misleading users.
% O’Brien and Lauer~\cite{o2018testing} find that people are still susceptible to deceptive visualization tactics, even when the visualizations are paired with accurate explanatory text. McNutt et al. devise strategies to detect ``visualization mirages''~\cite{mcnutt2020surfacing}, errors in the data or visualization design that may lead viewers to incorrect conclusions.

% A common theme in existing bias research is that the viewers may not always be cognizant of how visualizations influence their decision-making, but can nevertheless be biased by different design choices.
We seek to understand the impact of additional contextual information on users’ visualization preferences. However, we study this topic from the higher-level perspective of gauging trust in particular \emph{sources} of recommendations (i.e., human or algorithm).

\vspace{-0.5em}
%\vspace{-3mm}
\subsection{Algorithmic Decisions and Trust}
\label{sec:related-work:decisions-trust}

Several projects investigate how people respond to recommendations or decisions made by algorithms.
Victor et al.~\cite{victor2011trust} explain how users tend to trust recommendations from known entities (particularly people) more than unknown entities (i.e., complete strangers or algorithms); 
% Dietvorst et al.~\cite{dietvorst2015algorithm} find that users tend to avoid algorithms after witnessing them make mistakes, but this trust can be somewhat regained if users are able to modify the algorithm~\cite{jakesch2019ai}.
Lee~\cite{lee2018understanding} finds that users seem to distrust managerial decisions made by algorithms, due in part to a feeling of dehumanization by algorithms and a lack of shared social understanding. 
% Castelo et al.~\cite{castelo2019let} also observe that users tend to trust humans more than AI, in particular when tasks require subjectivity, and provide recommendations to increase user trust in AI-generated decisions. 
In contrast to the above studies that showcase negative responses to algorithmic decision-making, Logg et al.~\cite{logg} found that people were more likely to adhere to advice when they \highlight{believed} it was given by an algorithm than by a person. 
% Yang et al.~\cite{YangVisualExplanations} found that users' trust in classification algorithms could be increased through providing an explanation, even in the face of poor algorithmic performance. 
In situations where algorithmic performance is ambiguous (i.e., neither clearly good nor clearly poor), users' generalized implicit attitudes towards automation impact their propensity to trust a specific automated system~\cite {merrittAmbiguous}. These studies indicate that user trust in algorithmic decisions appears to be very situational in nature.


% Edwards et al.~\cite{edwards2014bot} find that Twitterbots are considered credible and competent communication agents, even when compared to human agents on Twitter.
% In the case of computer-generated versus human-written news articles, Graefe et al.~\cite{graefe2018readers} find that readers consistently prefer human-written articles.
% Shank~\cite{shank2013computers} studies how people perceive organizations when they interact with a human versus an automated representative and find that people perceive ``organizations as more responsible and in control when they have employed human, not computer, representatives''. Jakesch et al.~\cite{jakesch2019ai} find that people seem to trust renters on AirBnB more when they write their own profiles, compared to renters whose profiles are generated by AI; however, this effect is only observed when human-written and AI-generated profiles are placed side-by-side for comparison.

% A number of projects investigate situations where algorithms are used as communicators, and evaluate how people perceive those algorithmically-mediated interactions.
A number of projects evaluate people's perception of interactions with agents declared to be algorithmic or human, when in fact, the source is held constant. 
Shank~\cite{shank2013computers} finds that people perceive ``organizations as more responsible and in control when they have employed human, not computer, representatives.'' Jakesch et al.~\cite{jakesch2019ai} find that people seem to trust renters on \highlight{Airbnb} more when they write their own profiles compared to renters whose profiles \highlight{they believe} are generated by AI; however, this effect is only observed when human-written and AI-generated profiles are compared side-by-side. Graefe et al.~\cite{2016newscredibility} go one step further by modifying both the declared and \textit{actual} source of news articles (computer or human written). They find that while modifying the declared source had small but consistent effects in favor of human-written articles, modifying the actual source had larger effects. Participants generally regarded computer-written articles as more credible but less readable. 

We see many observations in the literature of users preferring interactions with, recommendations from, and unilateral decisions by humans over algorithms, with some exceptions (e.g., \cite{edwards2014bot}). However, no existing studies explicitly measure user trust in sources of recommendations for visual analytics, so it is unclear to what degree these results also apply to visualization. In this paper, we present a first step towards measuring user trust in human-curated versus algorithm-generated visualization recommendations.

% Thus, it is unclear whether these results also apply to visualization, despite the increasing popularity of ``automated'' visualization recommendation systems.

%and propose guidelines
